Emotion Recognition and Generation: A Comprehensive Review of Face, Speech, and Text Modalities

Emotion recognition and generation have emerged as crucial topics in Artificial Intelligence research, playing a significant role in enhancing human-computer interaction within healthcare, customer service, and other fields. Although several reviews have been conducted on emotion recognition and generation as separate entities, many of these works are either fragmented or limited to specific methodologies, lacking a comprehensive overview of recent developments and trends across different modalities. In this survey, we provide a holistic review aimed at researchers beginning their exploration in emotion recognition and generation. We introduce the fundamental principles underlying emotion recognition and generation across facial, vocal, and textual modalities. This work categorises recent state-of-the-art research into distinct technical approaches and explains the theoretical foundations and motivations behind these methodologies, offering a clearer understanding of their application. Moreover, we discuss evaluation metrics, comparative analyses, and current limitations, shedding light on the challenges faced by researchers in the field. Finally, we propose future research directions to address these challenges and encourage further exploration into developing robust, effective, and ethically responsible emotion recognition and generation systems.

==> datasets_table.tex <==

\begin{table}[H]
\small
\centering
\begin{tabular}{|p{3cm}|p{5cm}|p{2cm}|p{2cm}|p{3cm}|}
\hline
\textbf{Name} & \textbf{Description} & \textbf{Type} & \textbf{Size} & \textbf{Emotions} \\ \hline

AffectNet & Extensive facial imagery dataset annotated with discrete and continuous emotion labels. & Image & 450,000 images & Surprise, fear, disgust, happiness, sadness, anger, neutral, contempt \\ \hline

RAF-DB & Diverse facial expression dataset featuring multiple genders, ages, and ethnicities. & Image & 29,672 images & Surprise, fear, disgust, happiness, sadness, anger, neutral \\ \hline

FERPlus & Derived from the FER2013 dataset, enhancing expression annotations through crowdsourcing. & Image & Unlimited & Surprise, fear, disgust, happiness, sadness, anger, neutral, contempt \\ \hline

AFEW & High-resolution videos from YouTube with over 300 subjects and 10,000 sentences. & Video & 16 hours & Surprise, fear, disgust, happiness, sadness, anger, neutral \\ \hline

HDTF & Video clips gathered from TV shows and movies, including various head poses and occlusions. & Video & 1,809 clips & Surprise, fear, disgust, happiness, sadness, anger, neutral \\ \hline

AFEW-VA & Video clips annotated for valence and arousal levels, with 68 facial landmarks per frame. & Video & 600 clips & Surprise, fear, disgust, happiness, sadness, anger, neutral \\ \hline

DFEW & Facial expression dataset created from more than 1,500 movies. & Video & 12,059 clips & Happiness, anger, sadness, fear, disgust, surprise, neutral \\ \hline

CK+ & Laboratory-controlled video data capturing transitions from neutral to peak expression. & Video & 593 sequences & Surprise, fear, disgust, happiness, sadness, anger, contempt \\ \hline

MEAD & High-resolution emotional audiovisual dataset with 60 actors. & Video \& audio & 16,800 hours & Surprise, fear, disgust, happiness, sadness, anger, contempt \\ \hline

LRW & Video sequences of people speaking words in uncontrolled conditions. & Video \& audio & 1,000 utterances & Unlabeled \\ \hline

LibriTTS & Multi-speaker English corpus of read speech at 24kHz for TTS research. & Audio & 585 hours & Unlabeled \\ \hline

VCC2018 & Dataset for speech-to-speech systems, consisting of male and female speakers. & Audio & 464 sentences & Unlabeled \\ \hline

ESD & Collection of audio recordings for studying emotions expressed through speech. & Audio & 7,000 utterances & Neutral, happy, angry, sad, surprise \\ \hline

Empathetic Dialogues & Open-domain conversations between speakers and listeners for empathic responses. & Audio & 24,850 conversations & 32 emotion labels \\ \hline

EMO-DB & German emotional speech recorded by ten professional speakers. & Audio & 535 utterances & 7 emotions \\ \hline

CASIA & Mandarin emotional speech dataset. & Audio & 1,200 snippets & 6 emotions \\ \hline

Amazon Reviews & Large dataset of product reviews provided by Amazon. & Text & Unlimited & - \\ \hline

Twitter & Collection of tweets for social media text analysis. & Text & Unlimited & - \\ \hline

Reddit & Comments and posts from Reddit for understanding informal language. & Text & Unlimited & - \\ \hline

\end{tabular}
\caption{Datasets for ER and EG Systems}
\label{tab:datasets}
\end{table}

